Compact Distributed Certification of Planar Graphs

Naor, Parter, and Yogev (SODA 2020) have recently demonstrated the existence of a \emph{distributed interactive proof} for planarity (i.e., for certifying that a network is planar), using a sophisticated generic technique for constructing distributed IP protocols based on sequential IP protocols. The interactive proof for planarity is based on a distributed certification of the correct execution of any given sequential linear-time algorithm for planarity testing. It involves three interactions between the prover and the randomized distributed verifier (i.e., it is a \dMAM\/ protocol), and uses small certificates, on $O(\log n)$ bits in $n$-node networks. We show that a single interaction from the prover suffices, and randomization is unecessary, by providing an explicit description of a \emph{proof-labeling scheme} for planarity, still using certificates on just $O(\log n)$ bits. We also show that there are no proof-labeling schemes -- in fact, even no \emph{locally checkable proofs} -- for planarity using certificates on $o(\log n)$ bits.

==> lower-bound-bipartite.tex <==
% !TEX root = PLSPlanar.tex
Our proof is a (non-trivial) adaptation of the original lower bound proof for spanning tree and leader election, by G\"o\"os and Suomela~\cite{GoosS16}. We 
essentially follow the same steps, applying the necessary modifications in order to adapt the technique to our problem. Roughly speaking, we show that, if the certificates are of size $o(\log n)$, then it is possible to define a set of yes-instances (i.e., graphs not containing a $K_{p,q}$ as a minor) which can be \emph{glued} 
 together in order to obtain a no-instance (i.e., a graph containing a $K_{p,q}$ as a minor) in such a way that no vertex can distinguish to which instance it belongs. 


\begin{proposition}
There are no locally checkable proofs for $\mathrm{Forb}(\{ K_{p,q} \})$ using certificates on $o(\log n)$ bits,
for any $p \geq 2$ and $q \geq 3$.%\marginpar{\textcolor{red}{verifier valeurs k,p,q}}.
\end{proposition}

\begin{proof}
We begin supposing, by contradiction, that our problem admits a locally checkable proof with certificates of size $o(\log n)$. Without loss of generality, we assume that $q\geq p$, and in the following we also assume that $n \geq 6q$.

%As any graph containing $K_{p,p}$ as a minor also contains $K_{p,q}$ as a minor, for all $q\leq p$, we are going to show the lower-bound only of the case $p=q$.  

We start splitting the space of identifiers as in~\cite{GoosS16}. Let $n_A = \lfloor n/2 \rfloor$ and $n_B = \lceil n/2 \rceil$. Fix any partition of the identifiers $\{1, \dots, n^2\}$ into $2n$ subsets $a_1, \dots, a_n, b_1, \dots, b_n$ so that each $a \in A= \{a_1, \dots, a_n\}$ is of size $n_A$, and each $b\in  B = \{b_1, \dots, b_n\}$ is of size $n_B$. We denote by $a[i]$ (resp. $b[i]$) the $i$-th identifier of $a$ (resp.~$b$).

We now define a set of yes-instances $C(a,b)$ indexed by pairs $(a,b)\in A\times B$. Let $d = \lfloor n/(2q) \rfloor$. The instance $C(a,b)$ is defined by two disjoint paths, one of length $n_A$ and the other of length $n_B$. The first path contains the nodes $a$ in increasing order, while the second contains the nodes in $b$. Now, for each $i \in \{1, \dots, q\}$, make an edge between vertices $a[d \cdot i]$ and $b[d \cdot i]$. An example is shown in Figure \ref{fig:biplow1}.  

\begin{figure}[h]
\centering
\input{./figures/bipartite_lowerbound_1.tex}
\caption{Example of $C(a,b)$ when $n=22$, $p=q=3$, $d = 3$.}
\label{fig:biplow1}
\end{figure}

We claim that $C(a,b)$ is a yes-instance of our problem. Indeed, our graph is outerplanar and, therefore, it cannot contain a $K_{2,3}$ as a minor, nor any $K_{p,q}$ such that $p \geq 2$ and $q \geq 3$.

For each node $v\in V(C(a,b))$, let us call $P_{a,b}(v)$ the certificate that vertex $v$ receives on instance $C(a,b)$. Now define $$c(a,b) = \{P_{a,b}(a[d \cdot i]), P_{a,b}(b[d \cdot i]): i \in \{1, \dots, q\} \}.$$ 

In full words, $c(a,b)$ consists in all certificates from nodes $a[d \cdot i]$ and $b[d \cdot i]$, for all $i\in \{1, \dots, q\}$. Since we are assuming that each certificate is of size $o(\log n)$, we have that $c(a,b)$ contains $o(q\log n)$ bits. 

Now let $K_{n,n} = (A\cup B, E)$ be the complete bipartite graph with $E = \{\{a,b\}: a\in A, b\in B\}$. Each edge $\{a,b\}\in E$ is colored $c(a,b)$. Pick $n$ sufficiently large such that the number of bits of information in $c(a,b)$ is smaller than $\log(n)/(2q)$. This implies that there exists a subset of edges $F\subseteq E$ such that $|F| > |E|/n^{1/(2q)} = n^{2-1/(2q)}$ and all edges in $F$ have the same color. 

We now apply a result of  F{\"u}redi \cite{furedi1996upper}, which states that every graph having $n^{2-1/q} + o(n^{2-1/q})$ edges necessarily contains a $K_{q,q}$ as a subgraph. In particular this implies that for sufficiently large $n$ the graph $H=(A\cup B, F)$ contains a $K_{q,q}$ as a subgraph. Let us denote the vertices of this subgraph by $\tilde a_0, \dots, \tilde a_{q-1}$ and  $\tilde b_0, \dots, \tilde b_{q-1}$. As all edges of this complete bipartite graph have  the same color, we have that $c(\tilde a_{i_1}, \tilde b_{j_1}) = c(\tilde a_{i_2}, \tilde b_{j_2})$, for all $i_1, i_2, j_1, j_2 \in \{0, \dots, q-1\}$. 

We now create a new instance $W$, that roughly consists in gluing together the instances in order to construct a no-instance of our problem. We start creating $q$ copies of disjoint paths of length $n_A$ such that, in the $i$-th copy, we place the nodes of $\tilde a_{i-1}$ in increasing order. Similarly, we create $q$ copies of disjoint paths of length $n_B$, and in the $i$-th copy we place the nodes of $\tilde b_{i-1}$ in increasing order. Finally, for each $j \in \{0, \dots, q-1\}$ and each $i\in \{1, \dots, q\}$, add an edge between nodes $\tilde a_j[d \cdot i]$ and $\tilde b_{j+i}[d \cdot i]$, where the subindex $j+i$ is taken modulo $q$. See Figure \ref{fig:biplow2} for an example of the construction.  

\begin{figure}[h]
\centering
\input{./figures/bipartite_lowerbound_2.tex}
\caption{Example of graph $W$ for $p=q=3$ and $d = 3$.}
\label{fig:biplow2}
\end{figure}

We claim that $W$ is a no-instance of our problem. Indeed, observe that if we contract each disjoint path into a single node, and call the resulting nodes $v(\tilde a_0), \dots, v(\tilde a_{q-1}), v(\tilde b_0), \dots, v(\tilde b_{q-1})$, then the construction of $W$ implies that $v(\tilde a_i)$ is adjacent to $v(\tilde b_j)$, for all $i, j \in \{0, \dots, q-1\}$. We deduce that $K_{q,q}$ is a minor of $W$. This also implies that $K_{p,q}$ is a minor of $W$. 

Now consider the certificate where node $u \in W$ is such that that, when $u$ is a node in the path $\tilde a_j$ (resp. $\tilde b_j$), for $j\in \{0, \dots, q-1\}$, we give to $u$ the certificate that it would receive in $C(\tilde a_j, \tilde b_j)$. Observe that if $u$ is a node in $\tilde a_j$ (resp. $\tilde b_j$) that is different from $\tilde a_j[d \cdot i]$ (resp. $\tilde b_j[d \cdot i])$) for all $i \in \{1, \dots, q\}$, then $u$ does not distinguish whether it is in $W$ or in $C(\tilde a_j, \tilde b_j)$. Moreover, if $u$ equals  $\tilde a_j[d \cdot i])$ (resp. $\tilde b_j[d \cdot i])$)  for some $i \in \{1, \dots, q\}$, then the local neighborhood of $u$ looks exactly the same in both $W$ and $C(\tilde a_i,\tilde b_i)$. In all cases, all vertices accept the input $W$. Since $W$ is a no-instance, this contradicts the soundness of the protocol. We conclude that our problem does not admit a locally checkable proof of size $o(\log n)$. 

\end{proof}

\begin{remark}
The proof can also be generalized to the setting where the verifier can see at some constant distance $t$, by replacing each edge of the instances by a path of length $t$.
\end{remark}





==> lower-bound-clique.tex <==
% !TEX root = PLSPlanar.tex

\begin{proof}
The proof has the following structure.
We first define two similar types of instances that we call \emph{paths of blocks} and \emph{cycles of blocks}. 
We prove that paths of blocks are \emph{yes}-instances, that is they are $K_k$-minor-free, and that \emph{cycles of blocks} are \emph{no}-instance, that is, they contain $K_k$ as a minor. 
Finally, we show by combinatorial argument that if all the paths of blocks are accepted, and if the certificates used for these instances are too small, then there exists a cycle of blocks that is also accepted, which implies that the scheme is not correct. This implies the lower bound. This proof is inspired by the proof of Theorem~5 in~\cite{FeuilloleyH18}, which can be interpreted as the case $k=3$ (although it is not described for this problem in~\cite{FeuilloleyH18}). 

\subparagraph{Blocks and block connections}

Let $n=(k-1)(p+2)$, with $p$ an integer.
The instances we consider are made of \emph{blocks}. 
Consider a path on $k-1$ nodes, with identifiers $r(k-1),r(k-1)+1,..., (r+1)(k-1)-1$ in this order, for some integer $r \in [0,p+1]$. 
A block is such a path, where all the other edges have been added. 
In other words, a block is a $K_{k-1}$ with an ordering given by the identifiers. The block that starts with identifier $r\cdot(k-1)$ is called $B_{r}$.
There are two special blocks: $B_0$ is the \emph{starting block} and $B_{p+1}$ is the \emph{ending block}. The $p$ other blocks are called \emph{ordinary blocks}.
Note that the identifiers of the blocks are distinct.

We will now connect blocks by \emph{block connections}. A block connection, from  block $B_i$ to block $B_j$ is the following construction. Put the block $B_i$ with the nodes in increasing order on an horizontal line, and then to the right of it, put the block $B_j$, also with the nodes in increasing order. 
This gives an ordering from left to right to all the nodes.
Now add all edges between the $\lceil (k-1)/2 \rceil$ right most nodes of $B_i$  (which will be called the \emph{right part} of $B_i$) and the $\lfloor (k-1)/2 \rfloor$ left-most nodes of $B_j$ (which will be called the \emph{left  part} of $B_j$). See Fig.~\ref{fig:block-connexion}. 

\begin{figure}[htb]
\begin{center}
\input{figures/block-connection.tex}
\caption{Block connexion for $k=4$, from a block $B_i$ to a block $B_j$. Here $\lceil (k-1)/2 \rceil=2$ and $\lfloor (k-1)/2 \rfloor=1$, thus have two additional edges between the blocks.}
\label{fig:block-connexion}
\end{center}
\end{figure}

There are two important properties about these block connections.
First, two nodes that are linked by an edge have at most $k-3$ nodes between them in the horizontal ordering. In other words, no edge can \emph{jump} over more than $k-3$ nodes.
Second, if we connect $B_i$ to $B_j$ and $B_j$ to $B_k$, then, every node of $B_j$ is linked either to a node of $B_i$ or to a node of $B_k$ but not to both.  



\subparagraph{Two types of instances: path and cycles of blocks}
Now, given a permutation on $p$ elements, $\pi:p\rightarrow p$, we define a \emph{path of blocks}.
To create a path of blocks, we first take the starting block $B_0$ and then connect it to $B_{\pi^{-1}[1]}$. Then we continue and connect $B_{\pi^{-1}[1]}$ to $B_{\pi^{-1}[2]}$, etc. until we have finished the permutation. 
Finally, we connect $B_{\pi^{-1}[p]}$ with the ending block $B_{p+1}$.

A cycle of blocks is constructed in a similar way : let $\pi$ be a permutation and $k,  k'$ to integers such that $1 \leq k < k' \leq p$. A cycle of block is obtained, connecting   $B_{\pi^{-1}[ \ell ]}$ to $B_{\pi^{-1}[\ell +1]}$ for each $\ell$ with $ k \leq \ell < k'$,   and connecting $B_{\pi^{-1}[ k' ]}$ to $B_{\pi^{-1}[k]}$.  Hence, a cycle 
does not use the starting and ending blocks. 

Note that as the sets of the identifiers of the blocks are distinct, the paths and cycles are  well defined.

\subparagraph{Path of blocks are $K_k$-minor-free}
%It is easy to see that a path of blocks is free of $K_k$ as subgraphs. 
%Indeed, as noted earlier a path of blocks has edges that jump above at most $k-3$ nodes, and for a $K_k$ to appear we would need to have the first and the last nodes to be linked by an edge that jumps above at least $k-2$ nodes. 
%To show that a path of blocks is $K_k$-minor-free we need to show that even with edge contraction, we cannot make a $K_k$ appear.

By symmetry, there is no loss of generality in proving it  when $\pi$ is the identity permutation, and identifying agents withe identifiers.
The proof is easier if we add some edges,  assuming  that blocks are \emph{superconnected}, i.e. for $0 \leq r \leq p$,   each node $r(k-1) +i  $ of  $B_r$, with $0 \leq i \leq k-1$   is connected to all nodes $(r+1)(k-1) +j$  of  $B_{r+1}  $   such that $0 \leq j < i$.  
Notice that for each node $\ell$ the neighborhood of $v$ and $v$ itself  are the integers in the interval 
 $[ \ell -k+2, \ell +k -2] $. Thus, for each edge  $\{\ell, \ell'\}$, we have  $\vert \ell - \ell'  \vert \geq k-2$
 
 Hence  the  path of blocks is a subgraph of the new graph $G$  obtained by superconnection.  Thus, il  we prove that $G$ is $K_k$-minor-free,  then we are done.  

Suppose there is a $K_k$ minor in the graph $G$. Then there are $k$ disjoint sets of nodes such that: each set is connected, and for every pair $(S_i,S_j)$ of sets  $S_i \cup S_j $ is connected.
Let  $S_a$  be the last set met when nodes are successively explored according to the increasing order, let $\ell_a$ be the first node of $S_a$ in the increasing order. %,  and let $B_{r_a}$ be the block containing   $\ell_a$.   
Take a set $S_b$ such that  $S_b$ does not met the interval $[\ell_a- k+2,  \ell_a]$. Such a set exists because there are $k$ sets.   Let $\ell_b$ be a node of $S_b$ such that   $\ell_b < \ell_a$ . Such a node exists because $S_b$ is  met before $S_a$ where nodes are explored according to the increasing order. 

Consider the interval  $I =  [\ell_a- k+2,  \ell_a -1]$. Its contains   $k-2$ integers and $(S_a  \cup S_b ) \cap I$ is empty. Ir follows that  
$S_a  \cup S_b$ is not connected. Indeed there cannot exists an edge  $\{\ell, \ell'\}$ such that $\ell < \ell_a- k+2$ and
  $\ell' > \ell_a -1$ since $\vert \ell - \ell'  \vert \geq k-1$, and in the other hand $S_a  \cap ]\ell_a -1, (r+1)(p+2) ]$ and  $S_b  \cap [0, \ell_a -k+2[$ are both non-empty, since they respectively contain $\ell_a$  and $\ell_b$.  This contradicts the assumption that $S_a  \cup S_b$  is connected. 




%
%
%We have to cases according to  the place of $\ell_a$ in $B_{r_a}$. 
%
%\begin{itemize}
%\item if   $\ell_a$ is in  the left part of $B_{r_a}$, then $r_a \neq 0$ and  $\ell_a$ is connected  to the $\lceil (k-1)/2 \rceil$ right most nodes of $B_{r_a}$. Take a set $S_b$ such that  $S_b \neq S_a $,  and $S_b$ does not met the right part of $B_{r_a-1}$. Such a set exists because there are $k$ sets.   Let $\ell_b$ the the node of $S_b$   $\ell_b$ is before $\ell_a$  and there is no node of  $S_b$ between $\ell_b$ and $\ell_a$. Such a node exists because $S_b$ is  met before $S_a$ where nodes are explored according to the rank order. The node $\ell_b$ is either  the left  part  of $B_{r_a-1}$ or in a block $ B_r$ with $r < r_a -1$. 
%Thus,   $\ell_b$ has no neighbor in $\cup_{r \geq R_a} B_r $.   
%Now,  because of the minor definition there must exist a path from $\ell_a$ to $\ell_b$ using only nodes of $S_a$ and $S_b$. 
%
%
%\item if $\ell_a$ is in the right  $B_{r_a}$
%\end{itemize}

%
% successively explore 
%For every set $S_i$, let $\ell_i$ be the rank of the left-most node of $S_i$. 
%Let $S_a$ be the set for which $\ell_a$ is maximum. On its left, $\ell_a$ can be connected to nodes of at most $k-2$ other sets. Let $S_b$ be a set to which $\ell_a$ is not connected to its left. The set $S_b$ must have a node $u$ on the left of $\ell_a$ by definition, and this node has rank at most $\ell_a-(k-1)$ because it is not adjacent to $\ell_a$. Now because of the minor definition there must exist a path from $\ell_a$ to $u$ using only nodes of $S_a$ and $S_b$. 
%This path must contain an edge that jumps above $\ell_a$ and its $k-2$ left neighbors. But again this is impossible as the largest edges jump above at most $k-3$ nodes.


\subparagraph{Cycles of blocks are \emph{not} $K_k$-minor-free}

Consider a cycle of blocks, and distinguish an arbitrary block $B$. The instance without $B$ forms a connected set by construction. We contract this set into one node $v$. The node $v$ is connected to every node of $B$, because, as noted earlier, every node of $B$ was linked to at least one node outside of $B$. Now, as $B$ is $K_{k-1}$, the resulting graph is a $K_k$. 

\subparagraph{Cycles and paths of blocks are indistinguishable with small certificates}

Assume that there exists a scheme with certificates of size $g(n)=o(\log n)$. 
Then we claim that there exists two paths of blocks, where the prover gives to every block the exact same certificates in both paths of blocks.
Let a \emph{labeled block} be a block in which every node is given a label of size $g(n)$. For a given block, there are $2^{(k-1)f(n)}$ associated labeled blocks. Consider a set where we take one labeled version of each block. 
There are $2^{(k-1)g(n)p}$ such sets. 
On the other hand there are $p!$ different paths of blocks as there are $p!$ permutations of the ordinary blocks. 
We have:

\[
\log\left(2^{(k-1)g(n)p}\right) \in o(n\log n) 
\text{ and } 
\log(p!) \in \Omega(n\log n).
\]

Thus there are more paths of blocks than distinct sets of labeled blocks, thus by pigeon-hole principle, two paths of blocks should use the same labeled blocks. Let $A$ be the assignment of certificates to nodes that corresponds to this pair.

Now, without loss of generality, let us assume that one of paths of blocks corresponds to the identity permutation. The other permutation $\pi$ (as it is not the identity) must have two indices $i<j$ such that $\pi[i]>\pi[j]$. 
We can define a cycle of blocks $D$ the following way. Connect the blocks $B_i, B_{i+1},...,B_{j}$ in this order, and close the loop by connecting $B_{j}$ to $B_{i}$. 
We claim that in $D$ every node accepts if they are given the certificates described by $A$. Consider an arbitrary node in $D$, except the ones that have an edge in the connection from $B_{j}$ to $B_{i}$. This nodes has the exact same view as in the first labeled instance thus it accepts. Now consider a node that has an edge in the connection from $B_{j}$ to $B_{i}$. As noted earlier, such a node is not linked to a node from a third block. Thus it has the exact same view as in the second labeled instance.  
Then all the nodes of $D$ accept. 
This a contradiction because $D$ is a cycle of blocks, thus is a \emph{no}-instance: it contains a $K_k$.

It follows that $g(n)$ cannot be in $o(\log n)$ and the lower bound follows. 
\end{proof}

\begin{corollary}
For any finite family $\mathcal{F}$ of th form: $K_{k}\cup (\cup_{(a,b)\in S}K_{a,b})$ (where $S$ might be empty), the class of the graphs that exclude the graphs of $\mathcal{F}$ as minors, requires $\Omega(\log n)$ bits to be certified.
\end{corollary}

\begin{proof}
Let us show that the path of blocks considered in the proof above are $K_{2,2}$-minor-free, for any $k\geq 3$. 
Let us introduce some notations. 
In a \emph{yes}-instance, consider a node $v$ and its neighbors on its right. 
By construction these nodes are consecutive in the ordering, that is, they form an interval (where $v$ is the left endpoint).
Let this interval be $I_v$. 
We claim that two nodes $u$ and $v$ are connected if and only if $I_u \cap I_v \neq \emptyset$. 
Without loss of generality let $u<v$. 
If the nodes are connected, then $v$ is in the right neighborhood of $u$, thus $v \in I_u$, thus $v\in I_u \cap I_v$. 
On the other hand, if $I_u \cap I_v \neq \emptyset$ then, as $v$ is the left endpoint of $I_v$, necessarily, $v\in I_u$, thus $u$ and $v$ are connected.
This generalizes to connected sets of nodes. In particular, for a connected set of nodes~$S$, $I[S]=\cup_{u \in S} I[u]$ is also an interval. 
EQUIVALENCE

Now suppose that there is a $K_{2,2}$-minor. Note that $K_{2,2}$ is the cycle of length 4.
Let $S_i$ for $i\in [1,4]$ be the connected sets of nodes that are contracted to form the $K_{2,2}$, such that the cycle is $(1,2,3,4)$ with an edge between $1,4$.
Let $I_i=[a_i, b_i]$ be the associated intervals.
As $S_1$ and $S_3$ are not adjacent, $I_1$ and $I_3$ are disjoint, and without loss of generality, $b_1<a_3$. As $I_2$ and $I_4$ must both touch $I_1$ and $I_3$, $[b_1,a_3]$ must be contained in both, thus they intersect. But this is a contradiction: $S_2$ and $S_4$ should not be adjacent. 

Finally $K_{2,2}$-minor-freeness implies $K_{a,b}$-minor-freeness for any $a,b\geq 2$. Thus the path of blocks are in the class, and the cycles of blocks are not. The lower bound follows like above.
A CORRIGER
\end{proof}

\begin{corollary}
Planar graphs require $\Omega(\log n )$ bits to be certified.
\end{corollary}

This follows from the previous corollary with $\mathcal{F}=\{K_5,K_{3,3} \}$.
Note that this implies that the path of blocks with $k=5$ are actually planar. We provide a drawing of these instances in Fig. \ref{fig:planar-path-blocks}, because it is insightful. 

\begin{figure}[htb]
\begin{center}
\input{figures/planar-path-blocks.tex}
\end{center}
\caption{ Planar drawing of the paths of blocks for $k=5$. The construction is recursive. Start from the three left-most nodes and arrange them into a triangle. Then the fourth node is linked to the three first nodes, and we put it in the triangle. And then recursively, a node is always attached to at most the three nodes to its left, and these nodes from a triangular face. Note that with this construction can clearly not be adapted for a cycle of blocks: the more we go to the right the more edges there are to cross to be linked with node number 1.}
\label{fig:planar-path-blocks}
\end{figure}

\begin{remark}
The proof can be generalized to the setting where the verifier can see at some constant distance $t$, by replacing each edge of the instances by a path of length $t$.
\end{remark}


